Adaptive County Level COVID-19 Forecast Models: Analysis and Improvement

Accurately forecasting county level COVID-19 confirmed cases is crucial to optimizing medical resources. Forecasting emerging outbreaks pose a particular challenge because many existing forecasting techniques learn from historical seasons trends. Recurrent neural networks (RNNs) with LSTM-based cells are a logical choice of model due to their ability to learn temporal dynamics. In this paper, we adapt the state and county level influenza model, TDEFSI-LONLY, proposed in Wang et a. [l2020] to national and county level COVID-19 data. We show that this model poorly forecasts the current pandemic. We analyze the two week ahead forecasting capabilities of the TDEFSI-LONLY model with combinations of regularization techniques. Effective training of the TDEFSI-LONLY model requires data augmentation, to overcome this challenge we utilize an SEIR model and present an inter-county mixing extension to this model to simulate sufficient training data. Further, we propose an alternate forecast model, {\it County Level Epidemiological Inference Recurrent Network} (\alg{}) that trains an LSTM backbone on national confirmed cases to learn a low dimensional time pattern and utilizes a time distributed dense layer to learn individual county confirmed case changes each day for a two weeks forecast. We show that the best, worst, and median state forecasts made using CLEIR-Net model are respectively New York, South Carolina, and Montana.

==> Broader_Impact.tex <==
Two important steps in the medical resource supply chain are procurement and deployment. Each requires their own type of specialized forecasting tools. The power of this architecture described in this paper is it's ability to forecast over a large area cocurrently at a higher resolution and for less computational expense than existing models. The model can give healthcare administrators in charge of current medical resource allocation a two week lead time to deploy resources to where they are most needed. Meanwhile, we have found national trends to be easier to forecast as we would expect. For this reason, existing models are sufficient to forecast single dimension national or regional outputs and can reliably do so for periods longer than two weeks to the benefit of system administrators in charge of procurement who must predict national and regional resource demand.

%While the national stockpile managers and medical system resource procurers will care about national and regional forecasts which can be done over a longer time horizon using other forecasting tools. Those in charge of the deployment of existing medical resources need a model like this to cocurrently forecast cases at a county level in real time. These hospital system administrators can use this model to better inform their decisions with a two week lead time. 

%There is a role for both forecasting national and county trends. 

%Forecasting national trends can be used to forecast father into the future providing an accurate forecast of the U.S. demand for medical resources. These models say nothing of where these resources will be needed. The model in the paper serves the role of providing two week to the in charge of medical resource deployment. 

%We have found the forecasting of national trends to be easier due to the smaller noise to data ratio. This allows national forecasting models to be used on a longer time horizon than our county level model.




==> County_Selection.tex <==
\subsection{County Selection}
The estimation of highly populated and widely connected counties such as city hubs, which are arguably the most important to properly estimate, are systematically underestimated by the base model due to the influence of smaller less connected counties. To remedy this we can alter the loss function to avoid fitting the network to more isolated counties when analyzing these larger counties. This does however come at the trade off of overestimating the smaller counties. We observe this through minor or no increases to the mean square error, but a significant decrease to the population weighted mean square when employing county selection. Thus, we employ county selection as a method to get a more accurate prediction of larger counties at the expense of a less accurate prediction of smaller counties. Notably however, the overall accuracy stays relatively the same.

Naturally, highly populated, highly connected counties will have more influence on, and thus be more predictive of other counties. However, it is not the case that only highly populated counties are widely connected. Despite the aim being to predict highly populated counties, we do not want to omit highly connected counties without a large population, since these counties still provide valuable information for the estimation of the populated counties. Thus, a simple population based method would not suffice. Our approach is to determine a non-linear dependency between counties by calculating the mutual information (MI) between counties to determine a measure of how connected the county is. We then remove counties under a threshold, $\delta$.

To calculate the MI between a county, $C$, and another county $C'$, we estimate the MI of the two counties' time series of cases, denoted $t$ and $t'$, using the graph-based method, EDGE, proposed by \cite{mortezaetal2018}. Thus, in total we simply have:
\begin{equation}\begin{array}{cc}\label{eq.MI}
    I(C) = \rho(C, C') = EDGE(t, t')
\end{array}\end{equation}

However, we can not calculate the MI between every single county. It is simply too computationally expensive. Furthermore, intuitively it's obvious that there is lower dependency between counties that are far apart, therefore we compute MI between a county and its neighbors. To determine the neighbors of a county we use the county adjacency data provided by the United States Census Bureau. However, this could also easily be estimated using locations of counties. Nevertheless, this leaves us with a formulation for the average MI of a county, $C$. Let $k$ denote the number of neighboring counties $C'_i$ and we have:
\begin{equation}\begin{array}{cc}\label{eq.MI}
    \overline{I}(C) = \frac{1}{k}\sum_{i=1}^{k}\rho(C, C'_i)
\end{array}\end{equation}

Lastly. we normalize MI values using the formula $x = \frac{x - max(MI)}{max(MI) - min(MI)}$, and then remove counties with a normalized MI under the threshold $\delta$. Note that $\delta$ is our performance parameter and needs to be tuned. We tune $\delta$ by measuring the performance of the the network after training the network various values of $\delta$.

Algorithm 1 shows the implementation of this set up. The time series and neighboring county data for counties must be known beforehand. The output is a long mask.

\begin{algorithm}[H]
\SetAlgoLined
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{$\delta$ := Dependency Threshold\\
      Time series infection data for all counties\\
      Neighbor data for all counties\\}
\Output{Removed county mask\;}
\ForEach{County}{
    \ForEach{Neighbor}{
        $\rho$ = MI (County, Neighbor)\;
    }
   $\overline{\rho}$ = Average $\rho$\;
}
\BlankLine
\ForEach{\overline{\rho}}{
    $\overline{\rho}$ = $(\overline{\rho} - min(\overline{\rho})) / (min(\overline{\rho}) - max(\overline{\rho}))$\;
    \eIf{$\overline{\rho} < \delta$}{
        Set mask value to $0$\;
    }{
        Set mask value to $1$\;
    }
}
\caption{Dependency-based County Selection}
\end{algorithm}

\subsection{Delta Tuning}
We tune delta to optimize the population weighted mean square error of the model. It is important to note that county selection has minor impacts on the non-weighted MSE, and isn't used to reliably increase the overall accuracy of the model. We observe that as delta increases, the weighted MSE decreases up to an inflection point where it then starts increasing due to the loss of too much information. The non weighted MSE on the hand stays relatively the same, with a slight trend upwards. The optimization is done experimentally where we train the network at various delta values and compare the MSE and weighted MSE between them.

\begin{figure}[H]
    \centering
    \includegraphics[scale=0.6]{Figs/CountySelection/MSE_graph.png}
    \caption{Mean squared error and population weighted mean squared error at varying deltas. Note the steady decrease in weighted MSE compared to the small fluctuations observed in the MSE.}
    \label{fig:MSE_graph}
\end{figure}

Another thing to note in regards to county selection is the distribution of MI values. Most notably we observe a massive amount of counties at or near zero MI. The reason for the large number of counties at or near zero, is due to the significant number of counties that have little or no reported cases. We would expect zero mutual information to be calculated for these counties as a county with no cases during a widespread pandemic, must be isolated in some form. 

\begin{figure}[H]
    \centering
    \includegraphics[scale=0.75]{Figs/CountySelection/MI_distribution.png}
    \caption{Distribution of MI values. Note the large spike at zero. The distribution is relatively uniform apart from the beginning and end where it spikes heavily and drops off respectively.}
    \label{fig:MI_Distribution}
\end{figure}

Interestingly, this causes a massive amount of counties to be removed even at low pruning percentages. Despite this, the impact of county selection does not have an initial jump as one would expect at first.

\begin{table}[H]
\centering
\begin{tabular}{llll}
\multicolumn{1}{l}{$\delta$} & \multicolumn{1}{c}{Percentage of Removed Counties} &  \multicolumn{1}{c}{MSE} & \multicolumn{1}{c}{Weighted MSE} \\
\hline
\multicolumn{1}{l}{0}   & \multicolumn{1}{c}{0.00}      & \multicolumn{1}{c}{100715.3} & \multicolumn{1}{c}{2876.4} \\
\multicolumn{1}{l}{0.1} & \multicolumn{1}{c}{0.19}      & \multicolumn{1}{c}{100099.5} & \multicolumn{1}{c}{2819.7} \\
\multicolumn{1}{l}{0.2} & \multicolumn{1}{c}{0.27}      & \multicolumn{1}{c}{101607.6} & \multicolumn{1}{c}{2857.0} \\
\multicolumn{1}{l}{0.3} & \multicolumn{1}{c}{0.36}      & \multicolumn{1}{c}{100866.6} & \multicolumn{1}{c}{2432.3} \\
\multicolumn{1}{l}{0.4} & \multicolumn{1}{c}{0.45}      & \multicolumn{1}{c}{109388.3} & \multicolumn{1}{c}{2403.3} \\
\multicolumn{1}{l}{0.5} & \multicolumn{1}{c}{0.55}      & \multicolumn{1}{c}{101323.9} & \multicolumn{1}{c}{2372.3} \\
\multicolumn{1}{l}{0.6} & \multicolumn{1}{c}{0.65}      & \multicolumn{1}{c}{97567.3} & \multicolumn{1}{c}{1611.1} \\
\multicolumn{1}{l}{0.7} & \multicolumn{1}{c}{0.75}      & \multicolumn{1}{c}{106210.1} & \multicolumn{1}{c}{1393.2} \\
\multicolumn{1}{l}{0.8} & \multicolumn{1}{c}{0.85}      & \multicolumn{1}{c}{107970.5} & \multicolumn{1}{c}{1525.0} \\
\end{tabular}
\end{table}


==> Discussion_Conclusion.tex <==
\subsection{Adapted TDEFSI-based Model}
As is expected, adding regularization terms to the loss function of the TDEFSI model increased the final loss and MSE. However the regularization did improve the generalizability of the model, making it less likely to overfit the simulated training data. Using all the regularization methods discussed improved the model's ability to forecast county level data. However the forecasts on county level data was still significantly worse than the na{\"i}ve no-change benchmark. The forecast of the nationwide data was made worse by all the regularization except dropouts. Using only dropouts provided an improvement over the na{\"i}ve no-change benchmark for forecasting more than 4 days out.

While the TDEFSI models are viable for ILI forecasts as shown by \cite{Wangetal2020}, the minor adaptations to the TDEFSI-LONLY model tested here were insufficient to make the model a viable method for forecasting COVID-19 infection data. Since there exists no previous seasons of COVID-19 infections, the benefits of the novel two branch TDEFSI cannot be realized. More extreme adaptations or altogether different architectures must be considered to develop viable methods of forecasting COVID-19 data.

\subsection{Proposed RNN Architecture}

Consider smoothing using other forecasting techniques.

Sharing cell state between batches is essential to convergence.

Balance between capacity to fit complex observations and risk of over fitting. Many patterns superimposed on top of underlying pandemic dynamics such as state, local, or national level and temporal variation in policies for surveillance and social distancing.

\subsection{County Analysis}
The dependency measures of counties allows us to get a proxy measure for how connected a county is. Not only does this have a strong correlation with the accuracy of the network, but also the usage of the dependency measures have the potential to be applied in many other ways. The connections between counties is of course paramount when trying to analyze the spread of a pandemic.

\subsection{Conclusion}


==> Experiments.tex <==
\subsection{Na{\"i}ve No-Change Benchmark}
A na{\"i}ve approach to forecasting time-series data is to predict that there would be no change. This method provides a simple benchmark for evaluating the viability of a forecasting model. The forecasting methods described in this paper are used to forecast COVID-19 data for 5/18/2020 to 5/31/2020 based on the data from 1/22/2020 to 5/17/2020. The no-change benchmark used in the experiments forecasts that each the same as 5/17/2020. Figure \ref{fig:tdefsi_fc_nc} shows the MSE across all counties for each day in the na{\"i}ve no-change benchmark forecast. The bounds of $\pm\frac{1}{5}$ of the standard error for each experiment are also shown.  
\begin{figure}[H]
    \centering
    \includegraphics[width=0.5\textwidth]{Figs/TDEFSI/Forecast_nc.png}
    \caption{MSE of two week county forecast for na{\"i}ve no-change benchmark.}
    \label{fig:tdefsi_fc_nc}
\end{figure}
\subsection{Adapted TDEFSI-based Model} \label{sec:exp:tdefsi}
A total of 1024 SEIR simulations as described in Section \ref{SEIR} were run to train the TDFESI model as described in Section \ref{TDEFSI}, with an additional 16 simulations for validation. The network was trained for 300 epochs with a patience of 50. Four experiments were run with the TDFESI model. All the TDEFSI experiments were run on a 3.80GHz Intel i5-7600K processor with an NVIDIA RTX 2070 Super for GPU acceleration. Each epoch took an average of 320 seconds to complete. It was first trained without any regularization. Each experiment afterward added an additional regularization: dropouts with a rate of 0.1 between each layer, non-negative constraint regularization, and spacial consistency regularization. All experiments used the parameters $k = 2$, $H^{(i)} = 128$, $H = 256$, $\lambda = 0.01$, $\mu = 0.0001$ when relevant, which \cite{Wangetal2020} found to be optimal for their data. The final losses and MSE for each experiment are shown in Table \ref{tab:tdefsi_metrics}.

\begin{table}[H]
\centering
\caption{Results of training the TDEFSI-LONLY model with different regularization methods.}
\begin{tabular}{lrrrrr} 
\toprule
%& \multicolumn{4}{c}{Regularization Method} \\
& None & Dropout & Dropout \& $\delta(\widehat{z}_t)$ & Dropout \& $\delta(\widehat{z}_t)$ + $\phi(\widehat{z}_t)$ \\
\midrule
Train MSE & 2.57178e-5 & 5.24136e-5 & 1.54713e-4 & 2.444813e-4 \\
Valid MSE & 2.50214e-5 & 2.83442e-5 & 6.43349e-5 & 9.341941e-5 \\
Train Loss & - & - & 1.75519e-4 & 5.094754e-4 \\
Valid Loss & - & - & 8.26531e-5 & 1.906986e-4 \\
\bottomrule
\end{tabular}\label{tab:tdefsi_metrics}
\end{table}

Next the trained models were used to forecast on real COVID-19 data. The model was first input the nationwide totals for each day from 1/22/2020 to 5/17/2020. The final predicted nationwide total of the network was then fed back into the network as input to forecast additional days. The final 14 days of May were forecast and compared to the actual data. Figure \ref{fig:tdefsi_fc_mse} shows the MSE across all counties for each day in the forecast using each experiment. The bounds of $\pm\frac{1}{5}$ of the standard error for each experiment are also shown.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.75\textwidth]{Figs/TDEFSI/Forecast_MSE.png}
    \caption{MSE of two week county forecast for TDEFSI models.}
    \label{fig:tdefsi_fc_mse}
\end{figure}

Figure \ref{fig:tdefsi_fc_total} shows the absolute error of the predicted nationwide total for each day in the forecast using each experiment.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.75\textwidth]{Figs/TDEFSI/Forecast_Totals.png}
    \caption{Absolute error of two week nationwide total forecast for TDEFSI models.}
    \label{fig:tdefsi_fc_total}
\end{figure}
\iffalse
List of experiments:

{\bf RNN - Part I}:

\begin{itemize}
    \item TDEFSI LSTM on a large simulated dataset for Covid19, no tricks
    \item TDEFSI LSTM on a large simulated dataset for Covid19 with dropout
    \item TDEFSI LSTM on a large simulated dataset for Covid19 with dropout and non-negative regularization
    \item TDEFSI LSTM on a large simulated dataset for Covid19 with dropout, non-negative regularization, and spacial consistency regularization
    \item State outputs like NY, NJ, CA, ...
\end{itemize}
\fi
\subsection{Heirarchical Recurrent Time Distributed County Distributed Network (HDD)}\label{sec:exp:HDD}
\subsubsection{List of Experiments}
{\bf RNN - Part II}:
\begin{itemize}

    \item Network Capacity Varying $N_{LSTM}$ and $N_{DENSE}$ (done)
    \item Varying Forecast Horizon (1,7,14 days) (Maybe)
    \item Ablation Studies
        \begin{itemize}
            \item With the time distributed county level layer, and time distributed county distributed layer
            \item With the time distributed county level layer
            \item With the time distributed county distributed layer
        \end{itemize}
        
    \item Pretraining With Simulated Data (done)
    
\end{itemize}

The county level temporal patterns are supplemented by county level latitude, longitude, population, and population density as well as log(population) and log(population density) prior to the application of the county distributed dense layer which are standardized prior to training and inference. 

The model is trained with a batch size of 1, with batches taken in sequential order, and previous encoding cell state shared with the next batch. Sharing cell state between batches allows the model to make use of the memory property in the eponymous LSTM over the entire training period, without taking the gradient through long sequences. Each batch uses the vector of the previous end of day's recorded infections to forecast a target matrix of size $(N_{Counties}, N_{Days Forecast})$. 

The model is trained with features from the 1/22/20 to 5/2/20 period, targets from 1/23/20 to 5/16/20 with validation features from 1/22/20 to 5/4/20 and targets: 1/23/20 to 5/17/20. The trained model is tested by making a single 14 day forecast over 1/23/20 to 5/31/20 for all counties. 

Network parameters are optimized by minimizing the weighted mean squared error between the forecast and target matrices with NAdam with a learning rate of 0.001. Training is stopped when the validation loss is unimproved for 30 epochs at which weights from the best performing epoch are used for inference. 

Random dropout is applied to the targets during training at a rate of 0.25 to mitigate overfitting to any particular county's patterns. Light L1 and L2 regularization of 0.00005 are applied to the kernel and bias weights of all dense layers and to all recurrent weights to improve conditioning of the gradient\ref{bishop2006pattern}. 

Capacity experiments
The benefit of additional network capacity is explored by varying the number of features represented by the LSTM and by the final time/county distributed layer. 
-Too little=Underfitting, too much=Overfitting
-Averaging all predictions from the capacity experiments, slighltly improves



\begin{figure}[H]
    \centering
    \includegraphics[width=0.5\textwidth]{Figs/Heirarchical Recurrent Time Distributed County Distributed Model/Capacity Study.png}
    \caption{Mean Squared Error For Various Capacities and Configurations}
    \label{"BestWorstMedian"}
\end{figure}

In general, very small models, particularly with respect to temporal features, do not have enough capacity to well represent the complexity of the recorded infections data

\begin{figure}[H]
    \centering
    \includegraphics[width=0.5\textwidth]{Figs/Heirarchical Recurrent Time Distributed County Distributed Model/Capacity Experiment Training and Validation Traces.png}
    \caption{Training and Validation Curve For Individual Models and Averaged Across Models}
    \label{"BestWorstMedian"}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\textwidth]{Figs/Heirarchical Recurrent Time Distributed County Distributed Model/Best worst median forecasts.png}
    \caption{Best, Worst, and Median Forecasts of Ensemble Model Relative to No Change Benchmark.}
    \label{"BestWorstMedian"}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\textwidth]{Figs/Heirarchical Recurrent Time Distributed County Distributed Model/Best worst 5 state forecasts.png}
    \caption{Top 5 Best and Worst Forecasts Relative to No Change Benchmark.}
    \label{"BestWorst5"}
\end{figure}

\begin{tabular}{lrrrrr}
\toprule
      Model &            MSE &  Weighted MSE &  Total Parameters &  N\_LSTM &  N\_Dense \\
\midrule
       Average Ensemble of 20&   69870. &   2015. &               NaN &     NaN &      NaN \\
 14 day Naive Benchmark &  108276. &   3049. &               NaN &     NaN &      NaN \\
                     Best Scoring Single Model &   70905. &   2082. &           10945 &     2 &     24 \\
                     Median Scoring Single Model &   75707. &   2200. &           35847 &     9 &     34 \\
                     Worst Scoring Single Model &  188677. &   5662 &           24923 &     6 &     30 \\
\bottomrule
\end{tabular}





\begin{tabular}{lrrr}
\toprule
{} &  Na{\"i}ve Benchmark &  Variant 1 MSLE Objective &  Variant 1 MSE Objective \\
\midrule
Mean Squared Error             &       34190.0000 &                34095.0000 &               33727.0000 \\
Mean Squared Logarithmic Error &           0.0366 &                    0.0337 &                   0.0342 \\
Mean Absolute Error            &          28.9100 &                   28.4600 &                  27.3900 \\
Predicted Infection Increase   &           0.0000 &                 4279.0000 &               10024.0000 \\
\bottomrule
\end{tabular}

\begin{tabular}{lrr}
\toprule
{} &  Variant 2 MSLE Objective &  Variant 2 MSE Objective \\
\midrule
Mean Squared Error             &                 34102.000 &                14191.000 \\
Mean Squared Logarithmic Error &                     0.033 &                    1.149 \\
Mean Absolute Error            &                    28.400 &                   30.850 \\
Predicted Infection Increase   &                  4851.000 &               140971.000 \\
\bottomrule
\end{tabular}



{\bf County Selection}:
\begin{itemize}
    \item 
\end{itemize}

==> RNN.tex <==
Recurrent Neural Networks (RNNs) are suitable for our mission in this paper that is forecasting COVID-19 incident because they are able to learn temporal relationships. 
%Possibly the largest challenge in forecasting this novel disease is overcoming the curse of dimensionality with the limited data available. There is simply not enough data to justify a complex model with lots of parameters and explanatory features. One possible approach to handling this issue is using simulated data to supplement real data. Rather than optimizing the parameters of a detailed epidemiological model to fit the observed data, we can simulate many cases using randomized but relevant parameter sets. The results are then used to train an RNN model. 
\subsection{Adapted TDEFSI-based Model} \label{TDEFSI}
\def\btheta{\mathbf{\theta}}
\def\bz{\mathbf{z}}
\def\bx{\mathbf{x}}
\def\by{\mathbf{y}}
In this section we first recall TDEFSI model proposed in \cite{Wangetal2020} via transfer learning from simulated data generated from the proposed SEIR model introduced in Section \ref{pro.SEIR} to learn temporal relationships. TDEFSI model structure the output of the network at each step by including all counties, so that the network is able to learn spatial relationships, without requiring knowledge of specific relationships beforehand. Notations in \cite{Wangetal2020} are adapted to account for differences between ILI and COVID-19 data. Let $\by=(y_1,y_2,\ldots,y_T,\ldots)$ denote the sequence of the natural logs of daily nationwide incidence, where $y_t\in\mathbb{R}$. Let $\by^C=(\by_1^C,\by_2^C,\ldots,\by_T^C,\ldots)$ denote the sequence of daily incidence for a particular county $C\in\mathcal{D}$, where $\by_t^C\in\mathbb{R}^K$, where $K$ is the number of counties. The objective is defined as predicting both nationwide and county-level incidence at day $t$, where $t = T + 1$, denoted as $\bz_t=(y_t,\by^C_t)$. The TDEFSI loss function is given as:
\begin{equation} \label{eq:TLDR_loss}
    \min\limits_{\btheta} L(\btheta)=\diy\sum\limits_{t}\|\bz_t-\widehat{\bz}_t\|_2^2+\mu \phi(\widehat{\bz}_t) +\lambda\delta(\widehat{\bz}_t),
\end{equation}
where
\begin{itemize}
    \item $\phi(\widehat{\bz}_t)$: an activity regularizer added to the outputs for spatial consistency constraint
    \item $\delta(\widehat{\bz}_t)$: an activity regularizer added to the outputs for non-negative consistency constraint
\end{itemize}
Since RNNs are not affected by the temporal scale of its input sequence, (\ref{eq:TLDR_loss}) does not need to be adjusted to account for the fact that COVID-19 data is updated daily as opposed to the weekly ILI data. \cite{Wangetal2020} only considered ILI data for individual states and their counties, whereas for COVID-19 we consider all counties in the nation. Min-max normalization is used on the county-level data so that $\by^C\in[0,1]$. Whereas \cite{Wangetal2020} use the sum of $\by_t^C$ for $\by_t$, here $\by_t$ is the natural log of the sum of $\by_t^C$. This is done to normalize $\by_t$ relative to $\by_t^C$ while preserving the dependency of $\by_t$ on $\by_t^C$. Without this normalization, $\by_t$ would be significantly larger than $\by_t^C$ for a large $K$, and would dominate the gradients used to optimize (\ref{eq:TLDR_loss}). This modification to $\by_t$ requires that the regularization term $\phi(\widehat{\bz}_t)$ be modified to be
\begin{equation} \label{eq:TLDR_regularizer}
    \phi(\widehat{\bz}_t) =\lvert \exp{(\widehat{y}_t)} - \sum_{C\in \mathcal{D}}\widehat{y}_t^C \rvert.
\end{equation}
In Section \ref{sec:exp:tdefsi}, we use simulated data to supplement available real data and analyze the TDEFSI model. The architecture of the model used in these experiments is adapted specifically from the TDEFSI-LONLY model. This consists of $k$ LSTM layers, each with a latent dimension of $H^{(i)}$, followed by a dense layer with $H$ outputs, and a final dense layer with $K+1$ outputs. The input sequence to the network is $\by$, and the output sequence is $\widehat{\bz}$.

\iffalse % KL is not ready
However, due to effect of simulated data in the lost function we adding an extra regularization term to the loss function (\ref{eq:TLDR_regularizer}):
\begin{align} \label{eq:proposed_regularizer}
       \diy \min\limits_{\btheta} L(\btheta)=\sum\limits_{t}\|\bz_t-\widehat{\bz}_t\|_2^2+\mu \phi(\widehat{z}_t) +\lambda\delta(\widehat{z}_t)
             +\xi KL(p(\widehat{\bx}_n)\|p(\bx_n)),
\end{align}
where $KL(q(\widehat{\bx}_n)\|p(\bx_n))$ regularizer added to the outputs for simulated data, $q(\widehat{\bx}_n)$ is distribution of simulated data and $p(\bx_n)$ is distribution of original training data. 
The distributions $q(\widehat{\bx}_n)$ and $p(\bx_n)$ are approximated using Kernel Density Estimation [\cite{?}].

{\bf Steward: are we using weekly data? If not is it okay if we use the same lost function as TDEFSI?}. 
\fi
\subsection{Proposed RNN Architecture}


\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\textwidth]{Figs/Heirarchical Recurrent Time Distributed County Distributed Model/network diagram v2.png}
    \caption{Diagram of Hierarchical Recurrent Time Distributed County Distributed Network}
    \label{"HDD"}
\end{figure}






, linear layer, and dense layer as follows.

An alternative LSTM architecture, depicted in Fig. \ref{fig:altarchitecture}, represents a rethinking of the original TDEFSI architecture, designed to minimize the number of trainable parameters and more closely align with the underlying physical phenomenon. 

% David's description of the model
This architecture takes the cumulative sum of county confirmed cases at a given day as the input to an LSTM network which learns a general time-pattern. This time-pattern is distributed to an output linear dense layer with a number of units equal to the number of counties. This layer allows the model to scale the time-pattern for each county. Note the parameters in this layer are time distributed. each output of the linear dense layer is then used one at a time as one of seven features in a two hidden layer neural network with county distributed parameters to forecast the number of confirmed cases at the next day. The outputs of the the neural network then become the cumulative sum to serve as the input for the next days forecast. This architecture creates a hierarchy of features. The time-pattern takes priority over the population, latitude, longitude, population density, log pop, and log pop density features used in the neural network. The reduction in parameters comes from a combination of the LSTM network using only five dimensions as opposed to 128. In addition to the use of time distributed parameters in the output linear dense layer and the county distributed parameters in the neural network.(explain the conditional probability reasoning behind the features here) 

The primary features differentiating this architecture are the implementation of the skip connection adding the current number of infections to the output of each LSTM cell, the cumulative sumnation of the outputs of the LSTM cell, and the use of the hidden state of the previous batch's first LSTM cell to initialize the state of the same cell in the current batch. The skip connection and the cumulative sumnation force the network to learn the rate of change of the number of infections at each point. The use of the LSTM's stateful property to pass the hidden state from batch to subsequent batch allows the model to take advantage of it's internal memory between batches without using long input sequences. This enables the use of a smaller model trained will less data.

%{\bf Tyler: This section should be improved significantly as this is one of our major contributions in this paper. Please add more details about the proposed architecture and include the relevant formulas like input and output of each LSTM cell. We'll work on the diagram together once this part is done. }




%The input to this model is a single sum of county level cumulative confirmed cases at a day $t$. During training on John's Hopkins county level dataset the LSTM network captures the temporal trend of the national data and predicts a single national rate of change


%------------------------------------------
{\bf County Distributed Dense Layer:}\\
{\bf Time Distributed Linear Layer:}\\
{\bf Forecast LSTM:}\\

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{Figs/County Level Epidemiological Inference Recurrent Network (CLEIR-N)/network diagram v2.png}
%    \caption{Hierarchical Recurrent Time Distributed County Distributed Network}
\caption{County Level Epidemiological Inference Recurrent Network (CLEIR-Net). Cells with shared color have shared weights.}
    \label{fig:diagram}
\end{figure}

Denote the function of a standard LSTM cell, linear dense layer, and nonlinear dense layer as:

\begin{equation}
\langle h_i,C_i \rangle=L(h_{i-1},C_{i-1}|\theta),
\end{equation}

\begin{equation}
y=f(x|\theta),
\end{equation}

\begin{equation}
h=\phi(y|\theta).
\end{equation}
where $f$ and $\phi$ are linear and non-linear activation functions, respectively.

Let $t$ be the number of days elapsed since the first recorded national infection and let $I(t) \in \mathbb{Z}^{+^{N _{Counties}}}$ be the vector of true county level end of day infections. The encoder and remember LSTMs are given by:

\begin{equation}
\langle h_{-1},C^{(0)}(t) \rangle=L(\langle \sum(I(t)),t \rangle, C^{(0)}(t-1) |\theta_{Encode}), \qquad h,C \in \mathbb{R}^{N_{Time \ Features}}
\end{equation}

Where $N_{Time \ Features}$ is the number of features represented by the LSTM backbone. 

\begin{equation}
\langle h_0,C^{(1)}(t) \rangle=L(h_{-1}, C^{(1)}(t-1) |\theta_{Remember}).
\end{equation}

Let $i \in 1...N_{Forecast}$ be the index of the day in the forecast horizon. The extendable forecasting unit consists of a forecasting LSTM vertebrae, a time distributed linear layer, and a further time distributed/county distributed. The forecasting LSTM vertebrae is given by:

\begin{equation}
    \langle h_i,C^{(1)}(t+i) \rangle=L(h_{i-1}, C^{(1)}(t+i-1) |\theta_{Forecast}).
\end{equation}

The time distributed linear layer is then:

\begin{equation}
    h_i^{County}=f(h_i|\theta_{Time \ Distributed}), \qquad  h_i^{County} \in \mathbb{R}^{N_{Counties}}
\end{equation}

Let $X \in \mathbb{R}^{N_{Features} \times N_{Counties}}$ be an additional county level feature matrix and let $Z\in \mathbb{R}^{(N_{Features}+1) \times N_{Counties}}$ be the concatenation of $X$ with $h_i^{County}$ along the county axis, and let $j$ be the county index.The final layer predicts the change in each county's infections given it's current temporal feature through the following:

\begin{equation}
    \Delta I(t+i)_j=\phi(z_{j}|\theta_{County \ Distributed}), \qquad  \Delta I(t+i) \in \mathbb{R}^{N _{Counties}}.
\end{equation}

For $i \in 1...N_{Forecast}$, the forecast end of day recorded cases is then:

\begin{equation}
    \hat{I}(t+i)=\Delta I(t+i)+\hat{I}(t+i-1),
\end{equation}

and

\begin{equation}
    \hat{I}(t+1)=\Delta I(t+1)+I(t)
\end{equation}

for $i=1$.

The model has trainable parameters, 

$\theta_{E} \in (\mathbb{R}^{2 \times N_{TF}}, \ \mathbb{R}^{N_{TF} \times N_{TF}})$, 

$\theta_{R} \in (\mathbb{R}^{N_{TF} \times N_{TF}}, \ \mathbb{R}^{N_{TF} \times N_{TF}})$, 

$\theta_{F} \in (\mathbb{R}^{N_{TF} \times N_{TF}}, \ \mathbb{R}^{N_{TF} \times N_{TF}})$

$\theta_{TD} \in \mathbb{R}^{2 \times N_{C}}$, 

For the input, middle, and output layers of the County distributed dense layer.

$\theta_{CD} \in (\mathbb{R}^{(N_{F}+2) \times N_{D}}$, \ $\mathbb{R}^{(N_{D}+1) \times N_{D}}, \ \mathbb{R}^{(N_{D}+1) \times 1}$)



==> SEIR.tex <==
The most common extension of the SIR model for forecasting COVID-19 is SEIR which stands for {\textit Susceptible (S), Exposed (E), Infected (I), Recovered (R)}. As indicated in the acronym, this variant add a term to represent the latent population who are infected but have not yet become infectious themselves and assumes individuals gain immunity after recovery. This extension was chosen based on it's prevalence in the literature \cite{transmission_hubei,R_hubei,Hubei,Anastassopoulou2020}.The set of ordinary differential equations (ODEs) is defined by [\cite{SEIR}],neglecting birth and vaccination terms, and presented along with a conservation of population equation.
\def\diy{\displaystyle}
    \begin{align}\begin{array}{ccl}
      \diy \frac{dS}{dt} = - \beta\frac{ I S}{N}, \;\;\;
         \frac{dE}{dt}=\beta\frac{ I S}{N}-\sigma E,\;\;\;
         \frac{dI}{dt} = \sigma E - \gamma I, \;\;\;
         \frac{dR}{dt} = \gamma I,\\[10pt]
         N = S + E + I + R.
   \end{array} \end{align}

The parameters $\beta$, $\sigma$, and $\gamma$ control the rate of transition between labeled populations. In our SEIR generated data we chose a broad range of values that each parameter could take that would generate trends that increased both faster and slower than the JHU data. The generated data then uniformly samples the parameters within each range.

\subsection{Spatial Mixing Extension to SEIR by Incorporating Inter-County Flow}\label{pro.SEIR}


The mixing extension to the SEIR model is similar to the model described in Bonnasse et. al. \cite{bonnasse2018epidemiological}.\\
{\bf Notation:}
\vspace{-0.3cm}
\begin{itemize}
    \item $p_i$: Total population of county $i$, $i \in \{1,2,\ldots, N_{M}\}$, M is total number of counties.
     \item $p_{k,i}$: Population with status $k$ in county $i$, $k \in \{S,E,I,R\}$
     \item $x_{k,i}:=\diy p_{k,i}\big/p_i$
     \item $f_{i,j}$: Total population flow of people from county  $i$ to $j$ such that $f_{i,j}=f_{j,i}$ and $f_{i,i}=0$ for guaranteeing each county has no net change in population. 
\end{itemize}
Then the derivatives of $p_{k,i}$, $k \in \{S,E,I,R\}$ are defined by
\begin{equation}\begin{array}{l}
\diy \frac{d(p_{S,i}(t))}{dt}= \diy \sum_{j} f_{i,j} x_{S,j}- x_{S,i} \sum_{j} f_{j,i} - \beta_i p_{I,i}(t)  x_{S,i}(t), \\
\diy \frac{d(p_{E,i}(t))}{dt}= \sum_{j} f_{i,j} x_{E,j} - x_{E,i} \sum_{j} f_{j,i} + \beta_i p_{I,i}(t)  x_{S,i}(t) - \sigma p_{E,i}(t),\\
\diy\frac{d(p_{I,i}(t))}{dt}= \sum_{j} f_{i,j} x_{I,j} - x_{I,i} \sum_{j} f_{j,i} + \sigma p_{E,i}(t) - \gamma p_{I,i}(t),\\
\diy\frac{d(p_{R,i}(t))}{dt}= \sum_{j} f_{i,j} x_{R,j} - x_{R,i} \sum_{j} f_{j,i} + \gamma p_{I,i}(t).
\end{array}\end{equation}

For more compact form for efficient computation, let $\mathbf{F}^{bal}=\mathbf{F} - diag(\mathbf{1}^T \mathbf{F})$. The matrix $\mathbf{F}^{bal}$ has the important property that $\sum \mathbf{F}^{bal} \times \mathbf{1} = 0$, guaranteeing the conservation laws are satisfied. Then we have the following system of differential equations

\begin{equation}\begin{array}{l}
\diy \frac{d(\mathbf{p}_{S}(t))}{dt}= \mathbf{F}^{bal} \times \mathbf{x}_{S}(t) - \boldsymbol{\beta} \odot \mathbf{p}_{I}(t) \odot \mathbf{x}_{S}(t),\\
\diy \frac{d(\mathbf{p}_{E}(t))}{dt}= \mathbf{F}^{bal} \times \mathbf{x}_{E}(t) + \boldsymbol{\beta} \odot \mathbf{p}_{I}(t) \odot \mathbf{x}_{S}(t) - \sigma \mathbf{p}_{E}(t),\\
\diy \frac{d(\mathbf{p}_{I}(t))}{dt}= \mathbf{F}^{bal} \times \mathbf{x}_{I}(t) + \sigma \mathbf{p}_{E}(t) - \gamma \mathbf{p}_{I}(t),\\
\diy \frac{d(\mathbf{p}_{R}(t))}{dt}= \mathbf{F}^{bal} \times \mathbf{x}_{R}(t) + \gamma \mathbf{p}_{I}(t).
\end{array}\end{equation}
$\mathbf{p}_k(t)$ is then solved for iteratively using Euler's method [\cite{}].
\begin{equation}
\diy \mathbf{p}_k(t+h)=\mathbf{p}_k(t) + h \frac{d(\mathbf{p}_{k}(t))}{dt}, 
\end{equation}
where $h$ is learning parameters. Next assume that 
$$f_{i,j}= \diy \frac{\min(p_i,p_j)}{d_{i,j} \ \mu_{flow}}\;\;\hbox{and}\;\; \beta_i=\diy\frac{\rho_{i}}{\mu_{spread}},$$
where $d_{i,j}$ is the spatial distance between $i$ to $j$, $\rho_{i}$ is the population density of $i$, and, $\mu_{flow}$, $\mu_{spread}$ are the resistances to population flow, and infection spread respectively. The system is then controlled by the four parameters, $\mu_{flow}$, $\mu_{spread}$, $\sigma$, $\gamma$ and the initial conditions, which are estimated as follows 
\begin{equation}\begin{array}{ccl}
\diy p_{E,i}(0) \sim Possion(p_{i} \lambda_E), \;\; \; p_{I,i}(0) \sim Possion(p_{i} \lambda_E \lambda_I)\\[8pt]
p_{R,i}(0)=0, \;\;\; p_{S,i}(0)=p_{i}-p_{E,i}(0)-p_{I,i}(0),  
\end{array}\end{equation}
Where $\lambda_E$ and $\lambda_I$ represent the prevalence of exposure in the susceptible population, and the prevalence of infection in the exposed population at time zero, respectively. \\

%{\bf Tyler: Are all parts of the subsection 3.2 novel? If not we should cite relevant papers.}


